Flint for Safer Smart Contracts

The Ethereum blockchain platform supports the execution of decentralised applications or smart contracts. These typically hold and transfer digital currency to other parties on the platform; however, they have been subject to numerous attacks due to the unintentional introduction of bugs. Over a billion dollars worth of currency has been stolen since its release in July 2015. As smart contracts cannot be updated after deployment, it is imperative that the programming language supports the development of robust contracts. We propose Flint, a new statically-typed programming language specifically designed for writing robust smart contracts. Flint's features enforce the writing of safe and predictable code. To encourage good practices, we introduce protection blocks. Protection blocks restrict who can run code and when (using typestate) it can be executed. To prevent vulnerabilities relating to the unintentional loss of currency, Flint Asset traits provide safe atomic operations, ensuring the state of contracts is always consistent. Writes to state are restricted, simplifying reasoning about smart contracts.

==> soliditycontracts.tex <==
\section{Solidity Contracts}\label{soliditycontracts}

\subsection{The SimpleDAO}\label{Ssimple}

\begin{lstlisting}[language=Solidity, name=AppendixSDAO]

\end{lstlisting}

\subsection{The Multi-sig Wallet}\label{AppendixSWallet}

\begin{lstlisting}[language=Solidity, name=AppendixSwallet]

//sol Wallet
// Multi-sig, daily-limited account proxy/wallet.
// @authors:
// Gav Wood <g@ethdev.com>
// inheritable "property" contract that enables methods to be protected by requiring the acquiescence of either a
// single, or, crucially, each of a number of, designated owners.
// usage:
// use modifiers onlyowner (just own owned) or onlymanyowners(hash), whereby the same hash must be provided by
// some number (specified in constructor) of the set of owners (specified in the constructor, modifiable) before the
// interior is executed.

pragma solidity ^0.4.9;

contract WalletEvents {
  // EVENTS

  // this contract only has six types of events: it can accept a confirmation, in which case
  // we record owner and operation (hash) alongside it.
  event Confirmation(address owner, bytes32 operation);
  event Revoke(address owner, bytes32 operation);

  // some others are in the case of an owner changing.
  event OwnerChanged(address oldOwner, address newOwner);
  event OwnerAdded(address newOwner);
  event OwnerRemoved(address oldOwner);

  // the last one is emitted if the required signatures change
  event RequirementChanged(uint newRequirement);

  // Funds has arrived into the wallet (record how much).
  event Deposit(address _from, uint value);
  // Single transaction going out of the wallet (record who signed for it, how much, and to whom it's going).
  event SingleTransact(address owner, uint value, address to, bytes data, address created);
  // Multi-sig transaction going out of the wallet (record who signed for it last, the operation hash, how much, and to whom it's going).
  event MultiTransact(address owner, bytes32 operation, uint value, address to, bytes data, address created);
  // Confirmation still needed for a transaction.
  event ConfirmationNeeded(bytes32 operation, address initiator, uint value, address to, bytes data);
}

contract WalletAbi {
  // Revokes a prior confirmation of the given operation
  function revoke(bytes32 _operation) external;

  // Replaces an owner `_from` with another `_to`.
  function changeOwner(address _from, address _to) external;

  function addOwner(address _owner) external;

  function removeOwner(address _owner) external;

  function changeRequirement(uint _newRequired) external;

  function isOwner(address _addr) constant returns (bool);

  function hasConfirmed(bytes32 _operation, address _owner) external constant returns (bool);

  // (re)sets the daily limit. needs many of the owners to confirm. doesn't alter the amount already spent today.
  function setDailyLimit(uint _newLimit) external;

  function execute(address _to, uint _value, bytes _data) external returns (bytes32 o_hash);
  function confirm(bytes32 _h) returns (bool o_success);
}

contract WalletLibrary is WalletEvents {
  // TYPES

  // struct for the status of a pending operation.
  struct PendingState {
    uint yetNeeded;
    uint ownersDone;
    uint index;
  }

  // Transaction structure to remember details of transaction lest it need be saved for a later call.
  struct Transaction {
    address to;
    uint value;
    bytes data;
  }

  // MODIFIERS

  // simple single-sig function modifier.
  modifier onlyowner {
    if (isOwner(msg.sender))
      _;
  }
  // multi-sig function modifier: the operation must have an intrinsic hash in order
  // that later attempts can be realised as the same underlying operation and
  // thus count as confirmations.
  modifier onlymanyowners(bytes32 _operation) {
    if (confirmAndCheck(_operation))
      _;
  }

  // METHODS

  // gets called when no other function matches
  function() payable {
    // just being sent some cash?
    if (msg.value > 0)
      Deposit(msg.sender, msg.value);
  }

  // constructor is given number of sigs required to do protected "onlymanyowners" transactions
  // as well as the selection of addresses capable of confirming them.
  function initMultiowned(address[] _owners, uint _required) only_uninitialized {
    m_numOwners = _owners.length + 1;
    m_owners[1] = uint(msg.sender);
    m_ownerIndex[uint(msg.sender)] = 1;
    for (uint i = 0; i < _owners.length; ++i)
    {
      m_owners[2 + i] = uint(_owners[i]);
      m_ownerIndex[uint(_owners[i])] = 2 + i;
    }
    m_required = _required;
  }

  // Revokes a prior confirmation of the given operation
  function revoke(bytes32 _operation) external {
    uint ownerIndex = m_ownerIndex[uint(msg.sender)];
    // make sure they're an owner
    if (ownerIndex == 0) return;
    uint ownerIndexBit = 2**ownerIndex;
    var pending = m_pending[_operation];
    if (pending.ownersDone & ownerIndexBit > 0) {
      pending.yetNeeded++;
      pending.ownersDone -= ownerIndexBit;
      Revoke(msg.sender, _operation);
    }
  }

  // Replaces an owner `_from` with another `_to`.
  function changeOwner(address _from, address _to) onlymanyowners(sha3(msg.data)) external {
    if (isOwner(_to)) return;
    uint ownerIndex = m_ownerIndex[uint(_from)];
    if (ownerIndex == 0) return;

    clearPending();
    m_owners[ownerIndex] = uint(_to);
    m_ownerIndex[uint(_from)] = 0;
    m_ownerIndex[uint(_to)] = ownerIndex;
    OwnerChanged(_from, _to);
  }

  function addOwner(address _owner) onlymanyowners(sha3(msg.data)) external {
    if (isOwner(_owner)) return;

    clearPending();
    if (m_numOwners >= c_maxOwners)
      reorganizeOwners();
    if (m_numOwners >= c_maxOwners)
      return;
    m_numOwners++;
    m_owners[m_numOwners] = uint(_owner);
    m_ownerIndex[uint(_owner)] = m_numOwners;
    OwnerAdded(_owner);
  }

  function removeOwner(address _owner) onlymanyowners(sha3(msg.data)) external {
    uint ownerIndex = m_ownerIndex[uint(_owner)];
    if (ownerIndex == 0) return;
    if (m_required > m_numOwners - 1) return;

    m_owners[ownerIndex] = 0;
    m_ownerIndex[uint(_owner)] = 0;
    clearPending();
    reorganizeOwners(); //make sure m_numOwner is equal to the number of owners and always points to the optimal free slot
    OwnerRemoved(_owner);
  }

  function changeRequirement(uint _newRequired) onlymanyowners(sha3(msg.data)) external {
    if (_newRequired > m_numOwners) return;
    m_required = _newRequired;
    clearPending();
    RequirementChanged(_newRequired);
  }

  // Gets an owner by 0-indexed position (using numOwners as the count)
  function getOwner(uint ownerIndex) external constant returns (address) {
    return address(m_owners[ownerIndex + 1]);
  }

  function isOwner(address _addr) constant returns (bool) {
    return m_ownerIndex[uint(_addr)] > 0;
  }

  function hasConfirmed(bytes32 _operation, address _owner) external constant returns (bool) {
    var pending = m_pending[_operation];
    uint ownerIndex = m_ownerIndex[uint(_owner)];

    // make sure they're an owner
    if (ownerIndex == 0) return false;

    // determine the bit to set for this owner.
    uint ownerIndexBit = 2**ownerIndex;
    return !(pending.ownersDone & ownerIndexBit == 0);
  }

  // constructor - stores initial daily limit and records the present day's index.
  function initDaylimit(uint _limit) only_uninitialized {
    m_dailyLimit = _limit;
    m_lastDay = today();
  }
  // (re)sets the daily limit. needs many of the owners to confirm. doesn't alter the amount already spent today.
  function setDailyLimit(uint _newLimit) onlymanyowners(sha3(msg.data)) external {
    m_dailyLimit = _newLimit;
  }
  // resets the amount already spent today. needs many of the owners to confirm.
  function resetSpentToday() onlymanyowners(sha3(msg.data)) external {
    m_spentToday = 0;
  }

  // throw unless the contract is not yet initialized.
  modifier only_uninitialized { if (m_numOwners > 0) throw; _; }

  // constructor - just pass on the owner array to the multiowned and
  // the limit to daylimit
  function initWallet(address[] _owners, uint _required, uint _daylimit) only_uninitialized {
    initDaylimit(_daylimit);
    initMultiowned(_owners, _required);
  }

  // kills the contract sending everything to `_to`.
  function kill(address _to) onlymanyowners(sha3(msg.data)) external {
    suicide(_to);
  }

  // Outside-visible transact entry point. Executes transaction immediately if below daily spend limit.
  // If not, goes into multisig process. We provide a hash on return to allow the sender to provide
  // shortcuts for the other confirmations (allowing them to avoid replicating the _to, _value
  // and _data arguments). They still get the option of using them if they want, anyways.
  function execute(address _to, uint _value, bytes _data) external onlyowner returns (bytes32 o_hash) {
    // first, take the opportunity to check that we're under the daily limit.
    if ((_data.length == 0 && underLimit(_value)) || m_required == 1) {
      // yes - just execute the call.
      address created;
      if (_to == 0) {
        created = create(_value, _data);
      } else {
        if (!_to.call.value(_value)(_data))
          throw;
      }
      SingleTransact(msg.sender, _value, _to, _data, created);
    } else {
      // determine our operation hash.
      o_hash = sha3(msg.data, block.number);
      // store if it's new
      if (m_txs[o_hash].to == 0 && m_txs[o_hash].value == 0 && m_txs[o_hash].data.length == 0) {
        m_txs[o_hash].to = _to;
        m_txs[o_hash].value = _value;
        m_txs[o_hash].data = _data;
      }
      if (!confirm(o_hash)) {
        ConfirmationNeeded(o_hash, msg.sender, _value, _to, _data);
      }
    }
  }

  function create(uint _value, bytes _code) internal returns (address o_addr) {
    assembly {
      o_addr := create(_value, add(_code, 0x20), mload(_code))
      jumpi(invalidJumpLabel, iszero(extcodesize(o_addr)))
    }
  }

  // confirm a transaction through just the hash. we use the previous transactions map, m_txs, in order
  // to determine the body of the transaction from the hash provided.
  function confirm(bytes32 _h) onlymanyowners(_h) returns (bool o_success) {
    if (m_txs[_h].to != 0 || m_txs[_h].value != 0 || m_txs[_h].data.length != 0) {
      address created;
      if (m_txs[_h].to == 0) {
        created = create(m_txs[_h].value, m_txs[_h].data);
      } else {
        if (!m_txs[_h].to.call.value(m_txs[_h].value)(m_txs[_h].data))
          throw;
      }

      MultiTransact(msg.sender, _h, m_txs[_h].value, m_txs[_h].to, m_txs[_h].data, created);
      delete m_txs[_h];
      return true;
    }
  }

  // INTERNAL METHODS

  function confirmAndCheck(bytes32 _operation) internal returns (bool) {
    // determine what index the present sender is:
    uint ownerIndex = m_ownerIndex[uint(msg.sender)];
    // make sure they're an owner
    if (ownerIndex == 0) return;

    var pending = m_pending[_operation];
    // if we're not yet working on this operation, switch over and reset the confirmation status.
    if (pending.yetNeeded == 0) {
      // reset count of confirmations needed.
      pending.yetNeeded = m_required;
      // reset which owners have confirmed (none) - set our bitmap to 0.
      pending.ownersDone = 0;
      pending.index = m_pendingIndex.length++;
      m_pendingIndex[pending.index] = _operation;
    }
    // determine the bit to set for this owner.
    uint ownerIndexBit = 2**ownerIndex;
    // make sure we (the message sender) haven't confirmed this operation previously.
    if (pending.ownersDone & ownerIndexBit == 0) {
      Confirmation(msg.sender, _operation);
      // ok - check if count is enough to go ahead.
      if (pending.yetNeeded <= 1) {
        // enough confirmations: reset and run interior.
        delete m_pendingIndex[m_pending[_operation].index];
        delete m_pending[_operation];
        return true;
      }
      else
      {
        // not enough: record that this owner in particular confirmed.
        pending.yetNeeded--;
        pending.ownersDone |= ownerIndexBit;
      }
    }
  }

  function reorganizeOwners() private {
    uint free = 1;
    while (free < m_numOwners)
    {
      while (free < m_numOwners && m_owners[free] != 0) free++;
      while (m_numOwners > 1 && m_owners[m_numOwners] == 0) m_numOwners--;
      if (free < m_numOwners && m_owners[m_numOwners] != 0 && m_owners[free] == 0)
      {
        m_owners[free] = m_owners[m_numOwners];
        m_ownerIndex[m_owners[free]] = free;
        m_owners[m_numOwners] = 0;
      }
    }
  }

  // checks to see if there is at least `_value` left from the daily limit today. if there is, subtracts it and
  // returns true. otherwise just returns false.
  function underLimit(uint _value) internal onlyowner returns (bool) {
    // reset the spend limit if we're on a different day to last time.
    if (today() > m_lastDay) {
      m_spentToday = 0;
      m_lastDay = today();
    }
    // check to see if there's enough left - if so, subtract and return true.
    // overflow protection                    // dailyLimit check
    if (m_spentToday + _value >= m_spentToday && m_spentToday + _value <= m_dailyLimit) {
      m_spentToday += _value;
      return true;
    }
    return false;
  }

  // determines today's index.
  function today() private constant returns (uint) { return now / 1 days; }

  function clearPending() internal {
    uint length = m_pendingIndex.length;

    for (uint i = 0; i < length; ++i) {
      delete m_txs[m_pendingIndex[i]];

      if (m_pendingIndex[i] != 0)
        delete m_pending[m_pendingIndex[i]];
    }

    delete m_pendingIndex;
  }

  // FIELDS
  address constant _walletLibrary = 0xcafecafecafecafecafecafecafecafecafecafe;

  // the number of owners that must confirm the same operation before it is run.
  uint public m_required;
  // pointer used to find a free slot in m_owners
  uint public m_numOwners;

  uint public m_dailyLimit;
  uint public m_spentToday;
  uint public m_lastDay;

  // list of owners
  uint[256] m_owners;

  uint constant c_maxOwners = 250;
  // index on the list of owners to allow reverse lookup
  mapping(uint => uint) m_ownerIndex;
  // the ongoing operations.
  mapping(bytes32 => PendingState) m_pending;
  bytes32[] m_pendingIndex;

  // pending transactions we have at present.
  mapping (bytes32 => Transaction) m_txs;
}

contract Wallet is WalletEvents {

  // WALLET CONSTRUCTOR
  //   calls the `initWallet` method of the Library in this context
  function Wallet(address[] _owners, uint _required, uint _daylimit) {
    // Signature of the Wallet Library's init function
    bytes4 sig = bytes4(sha3("initWallet(address[],uint256,uint256)"));
    address target = _walletLibrary;

    // Compute the size of the call data : arrays has 2
    // 32bytes for offset and length, plus 32bytes per element ;
    // plus 2 32bytes for each uint
    uint argarraysize = (2 + _owners.length);
    uint argsize = (2 + argarraysize) * 32;

    assembly {
      // Add the signature first to memory
      mstore(0x0, sig)
      // Add the call data, which is at the end of the
      // code
      codecopy(0x4,  sub(codesize, argsize), argsize)
      // Delegate call to the library
      delegatecall(sub(gas, 10000), target, 0x0, add(argsize, 0x4), 0x0, 0x0)
    }
  }

  // METHODS

  // gets called when no other function matches
  function() payable {
    // just being sent some cash?
    if (msg.value > 0)
      Deposit(msg.sender, msg.value);
    else if (msg.data.length > 0)
      _walletLibrary.delegatecall(msg.data);
  }

  // Gets an owner by 0-indexed position (using numOwners as the count)
  function getOwner(uint ownerIndex) constant returns (address) {
    return address(m_owners[ownerIndex + 1]);
  }

  // As return statement unavailable in fallback, explicit the method here

  function hasConfirmed(bytes32 _operation, address _owner) external constant returns (bool) {
    return _walletLibrary.delegatecall(msg.data);
  }

  function isOwner(address _addr) constant returns (bool) {
    return _walletLibrary.delegatecall(msg.data);
  }

  // FIELDS
  address constant _walletLibrary = 0xcafecafecafecafecafecafecafecafecafecafe;

  // the number of owners that must confirm the same operation before it is run.
  uint public m_required;
  // pointer used to find a free slot in m_owners
  uint public m_numOwners;

  uint public m_dailyLimit;
  uint public m_spentToday;
  uint public m_lastDay;

  // list of owners
  uint[256] m_owners;
}

\end{lstlisting}

\subsection{King of the Ether Throne}\label{AppendixSKing}

\begin{lstlisting}[language=Solidity, name=AppendixSking]
pragma solidity ^0.4.2;

contract KotET {
  address public king;
  uint public claimPrice = 100;
  address owner;

  function KotET() {
    owner = msg.sender;
    king = msg.sender;
    if (msg.value<1 ether) throw;
  }

  function sweepCommission(uint amount)  {
    bool res = owner.send(amount);
  }

  function() payable {
    if (msg.value < claimPrice) throw;

    uint compensation = calculateCompensation();
    bool res = king.send(compensation);
    king = msg.sender;
    claimPrice = calculateNewPrice();
  }

  function calculateCompensation() private returns(uint) {
    return claimPrice+100;
  }

  function calculateNewPrice() private returns(uint) {
    return msg.value+200;
  }
}

contract KotET2 {
  address public king;
  uint public claimPrice = 100;
  address owner;

  function KotET2() {
    owner = msg.sender;
    king = msg.sender;
  }

  function sweepCommission(uint amount)  {
    bool res = owner.send(amount);
  }

  function() payable {
    if (msg.value < claimPrice) throw;

    uint compensation = calculateCompensation();
    if (!king.call.value(compensation)()) throw;
    king = msg.sender;
    claimPrice = calculateNewPrice();
  }

  function calculateCompensation() private returns(uint) {
    return claimPrice+100;
  }

  function calculateNewPrice()  private returns(uint) {
    return claimPrice+200;
  }
}

contract Bob {
  uint public count;

  function unseatKing(address king, uint w){
    bool res = king.call.value(w)();
  }

  function() payable{
    count++;
  }
}

contract Mallory {

  function unseatKing(address king, uint w){
    bool res = king.call.value(w)();
  }

  function() payable {
    throw;
  }
}

\end{lstlisting}

\subsection{Proof of Weak Hands Coin}\label{AppendixCoin}

\begin{lstlisting}[language=Solidity, name=Appendixcoin]
// Cutdown PonziToken to just show vulnerability

pragma solidity ^0.4.11;

contract PonziToken {
	uint256 public totalSupply;
	// amount of shares for each address (scaled number)
	mapping(address => uint256) public balanceOf;
	// allowance map, see erc20
	mapping(address => mapping(address => uint256)) public allowance;

	function PonziToken() {
		owner = msg.sender;
	}

	function transferFrom(address _from, address _to, uint256 _value) {
      var _allowance = allowance[_from][msg.sender];
      if (_allowance < _value)
          throw;
      allowance[_from][msg.sender] = _allowance - _value;
      transferTokens(_from, _to, _value);
  }

	function transferTokens(address _from, address _to, uint256 _value) internal {
		if (balanceOf[_from] < _value)
			throw;
		if (_to == address(this)) {
			sell(_value);
		} else {
		    // Omitted as not relevant to vulnerability
		}
	}

	function sell(uint256 amount) internal {
		// remove tokens
		totalSupply -= amount;
		balanceOf[msg.sender] -= amount;
	}
}

\end{lstlisting}


